EMFormer: Efficient Multi-Scale Transformer for Accumulative Context Weather Forecasting

Long-term weather forecasting is critical for socioeconomic planning and disaster preparedness. While recent approaches employ finetuning to extend prediction horizons, they remain constrained by the issues of catastrophic forgetting, error accumulation, and high training overhead. To address these limitations, we present a novel pipeline across pretraining, finetuning and forecasting to enhance long-context modeling while reducing computational overhead. First, we introduce an Efficient Multi-scale Transformer (EMFormer) to extract multi-scale features through a single convolution in both training and inference. Based on the new architecture, we further employ an accumulative context finetuning to improve temporal consistency without degrading short-term accuracy. Additionally, we propose a composite loss that dynamically balances different terms via a sinusoidal weighting, thereby adaptively guiding the optimization trajectory throughout pretraining and finetuning. Experiments show that our approach achieves strong performance in weather forecasting and extreme event prediction, substantially improving long-term forecast accuracy. Moreover, EMFormer demonstrates strong generalization on vision benchmarks (ImageNet-1K and ADE20K) while delivering a 5.69x speedup over conventional multi-scale modules. Code: https://github.com/chenhao-zju/emformer

==> sections/relatedwork.tex <==
\section{Related work}
\label{sec:related}


\subsection{Data-Driven Weather Forecasting}

Before the advent of data-driven methods, numerical weather prediction (NWP) was the predominant approach, producing forecasts by solving partial differential equations on high-resolution global grids~\cite{nwp, lynch2008origins, kalnay2002atmospheric}. While these methods deliver physically consistent and rigorously validated forecasts~\cite{molteni1996ecmwf, ritchie1995implementation}, they remain computationally prohibitive, especially at fine spatial scales.

The availability of large-scale atmospheric reanalysis datasets has since catalyzed a shift toward data-driven weather forecasting. Early exemplars such as FourCastNet~\cite{fourcastnet} and Pangu-Weather~\cite{panguweather} employed Fourier Neural Operators (FNO)~\cite{fno} and 3D Swin Transformers~\cite{liu2021swin}, respectively, to approximate atmospheric evolution. Subsequent research has largely bifurcated into two streams: (i) neural operators, including KNO~\cite{koopmanlab} and SFNO~\cite{sfno}, that directly learn the temporal evolution operator; and (ii) neural network, such as FengWu~\cite{fengwu}, GraphCast~\cite{graphcast}, FuXi~\cite{fuxi}, GenCast~\cite{gencast}, Stormer~\cite{stormer}, OneForecast~\cite{oneforecast}, and VAMoE~\cite{vamoe}, which incorporate inductive biases tailored to atmospheric dynamics. Both categories achieve competitive forecast skill with substantially lower computational cost.

Notably, FengWu-ghr~\cite{han2024fengwu} addresses error accumulation by adopting a Low-Rank Adaptation (LoRA) finetuning strategy that assigns distinct parameters to different forecast time steps. While this approach can mitigate error drift, it introduces additional overhead from loading and saving multiple model states. In contrast, our method employs KV-cache finetuning, which shares the same parameters across all time steps and reduces error accumulation by retaining key-value caches from previous steps, thereby avoiding unnecessary computational complexity.


% Before the booming of Data-driven methods, numerical weather prediction (NWP) prevailed, producing forecasts by solving PDEs on high-resolution global grids~\cite{nwp, lynch2008origins, kalnay2002atmospheric}. These methods deliver physically analysis and rigorously validated forecasts~\cite{molteni1996ecmwf, ritchie1995implementation}, but their computation remains prohibitively high, especially at fine scales.

% The emergence of large-scale atmospheric reanalyses has catalysed a shift toward data-driven forecasting. Early exemplars, FourCastNet~\cite{fourcastnet} and Pangu-Weather~\cite{panguweather}, employ Fourier Neural Operators (FNO)~\cite{fno} and 3D Swin Transformers~\cite{liu2021swin}, respectively, to approximate atmospheric evolution. Subsequent research has bifurcated into two streams: (i) neural operators, such as KNO~\cite{koopmanlab} and SFNO~\cite{sfno}, that directly learn the temporal evolution operator; and (ii) neural networks, including FengWu~\cite{fengwu}, GraphCast~\cite{graphcast}, FuXi~\cite{fuxi}, GenCast~\cite{gencast}, Stormer~\cite{stormer}, and VAMoE~\cite{vamoe}, which leverage inductive biases tailored to atmosphere. All achieve competitive skill with limited computation.

% Apart from this work, another work that tries to solve the error accumulation issue is FengWu-ghr~\cite{han2024fengwu}, which adopts a LoRA finetuning strategy to allocate different parameters to various time-steps. Although treating different time-steps with different model can avoid error accumulation, the model loading and saving take the extra complexity. In contrast, our KV-cache finetuning shares the same parameters during all the time-steps, and avoids error accumulation by remembering the KV-caches in the previous time-steps.


% Inspired by the success of MoE in LLMs~\cite{moe}, recent studies have begun to integrate MoE into weather forecasting. VAMoE~\cite{vamoe} extends MoE to incremental weather forecasting; EWMoE~\cite{ewmoe} augments FourCastNet with MoE layers. In contrast, we propose TMoE that explicitly partitions atmospheric inputs by month and dynamically routes them to specialized temporal experts. This structure enables STMoE to capture inter-month variability and intra-month correlation.




\subsection{KV Cache}

The emergence of Large Language Models (LLMs) has catalyzed the development of KV-cache techniques designed to improve context consistency and expedite long-context inference. Existing methods can largely be categorized into two main approaches: one employs dynamic sparse attention masks to bypass certain computations~\cite{dsflashattn, dota, ecsa, spatten}, while the other selectively discards portions of the KV cache based on characteristics of the input sequence~\cite{NEURIPS2023_cdaac2a0, pmlr-v202-sheng23a, ge2024model}. Both approaches have demonstrated success in extending the reasoning length and reducing computational complexity.

Building on these advances, recent research has extended KV-cache compression techniques to long-term video generation, giving rise to three prominent paradigms: training-free KV-cache compression~\cite{yi2025deep, kim2025infinipotv}, efficient compression using sparse attention matrices~\cite{zhang2025spargeattention, zhang2025clusterattn}, and dual-model architectures that separate memory and generation modules~\cite{zhu2025memorize}. These strategies have proven effective in accelerating video generation while enhancing temporal consistency.

Expanding the scope beyond LLMs and video generation, this work introduces a novel application of a KV-cache in long-term weather forecasting. By integrating autoregressive with this mechanism, our method preserves long-term context consistency while mitigating error accumulation.



% From the booming of Large Language Model(LLM), many works have been exploring the KV-Cache techniques to improve context consistency and accelerate the long-context LLM inference. The mainstream techniques can be divided into two paths, one of which is skipping computations with dynamic sparse attention masks~\cite{dsflashattn, dota, ecsa, spatten}, another is discarding KV cache based on the input sequence~\cite{NEURIPS2023_cdaac2a0, pmlr-v202-sheng23a, ge2024model}. Those two paths both successfully increase the reasoning length and reduce the computation complexity.

% Since the booming of KV cache compression in the long context inference, some recent works try to introduce the KV cache memory module to long-term video generation. There are three paradigms behind this technique, including training-free KV cache compression~\cite{yi2025deep, kim2025infinipotv}, efficient compression based on sparse attention matrix~\cite{zhang2025spargeattention, zhang2025clusterattn}, and dual-model architecture of memory and generation~\cite{zhu2025memorize}. Those methods are all make sense in accelerating video generation and increasing the temporal consistency.

% Apart from LLM and video generation, this work is the pioneer to introduce the KV cache memory module to long-term weather forecasting. By integrating the autoregressive method with memory module, this work can achieve long context consistency with low error accumulation.




